A Deep Reinforcement Learning Approach for Service Migration in MEC-enabled Vehicular Networks

Multi-access edge computing (MEC) is a key enabler to reduce the latency of vehicular network. Due to the vehicles mobility, their requested services (e.g., infotainment services) should frequently be migrated across different MEC servers to guarantee their stringent quality of service requirements. In this paper, we study the problem of service migration in a MEC-enabled vehicular network in order to minimize the total service latency and migration cost. This problem is formulated as a nonlinear integer program and is linearized to help obtaining the optimal solution using off-the-shelf solvers. Then, to obtain an efficient solution, it is modeled as a multi-agent Markov decision process and solved by leveraging deep Q learning (DQL) algorithm. The proposed DQL scheme performs a proactive services migration while ensuring their continuity under high mobility constraints. Finally, simulations results show that the proposed DQL scheme achieves close-to-optimal performance.

==> Sections/3_problem.tex <==
\subsection{Problem Formulation}
The problem is a multi-objective optimization problem where the aim is to optimize the communication delay, the computing delay as well as the migration costs. We transform the multi-objective problem into a single objective one by introducing the weights $\lambda_i$ for $i\in\{1,2,3\}$. The formulated problem is written as a nonlinear integer program (NLP) as follows. 

\begin{problem}\label{pb:1}
  \begin{alignat}{2} &\Minimize_{\mathbf{x}}&\qquad&\lambda_1C(\mathbf{x})+\lambda_2D(\mathbf{x})+\lambda_3M(\mathbf{x})\label{obj:1}\\
  & \subjto
  & & x_{i}^k(t)\in\{0,1\}, \quad \forall i,k,t, \label{C:def1}\\
  & & & \sum_{i=1}^{N}x_{i}^k(t)=1, \quad \forall k,t, \label{C:oneMEC}
 \end{alignat}
\end{problem}

The computing delay $C(\mathbf{x})$ is defined as follows:
\begin{align}\label{comput_delay}
    C(\mathbf{x})\coloneqq\sum_{i=1}^N\sum_{k=1}^K\sum_{t=1}^Tx_{i}^k(t)n_i(t)\frac{c^k(t)}{f_i},
\end{align}
where $c^k(t)$ denotes the required amount of computing capacity in CPU cycles of service $k$ at time-slot $t$ and $f_i$ denotes the maximum computing capacity of MEC node $i$ (in CPU cycles per second). The term $n_i(t)$ denotes the number of services placed at MEC node $i$, i.e.,
\begin{align}\label{num_services}
    n_i(t)\coloneqq\sum_{k=1}^Kx_{i}^k(t).
\end{align}

The communication delay $D(\mathbf{x})$ is defined as follows:
\begin{align}\label{commun_delay}
    D(\mathbf{x})\coloneqq\sum_{i=1}^N\sum_{k=1}^K\sum_{t=1}^Tx_{i}^k(t)d_i^k(t),
\end{align}
where $d_i^k(t)$ characterizes the general communication delay between MEC node $i$ and a user when its corresponding service $k$ is placed on MEC node $i$ at time-slot $t$. It mainly depends on the link bandwidth between the MEC node and the user and the amount of data transferred to the user. We use a general temr $d_i^k(t)$ to make our problem generic and independent to a specific transmission model.

Finally, the migration cost $M(\mathbf{x})$ is defined as follows:
\begin{align}\label{mig_cost}
    M(\mathbf{x})\coloneqq\sum_{i=1}^N\sum_{i'=1}^N\sum_{k=1}^K\sum_{t=1}^Tx_{i'}^k(t-1)x_i^k(t)m_{i'i}^k(t),
\end{align}
where the migration cost $m_{i'i}^k(t)$ is used to denote the cost of migrating the service $k$ from MEC node $i'$ to MEC node $i$. This costs includes bandwidth costs incurred by cross-edge migration (e.g., wide-area network bandwidth costs) as well as energy costs caused by increased energy consumption of network devices such as routers. To make the model general, we use the general term $m_{i'i}^k(t)$ as done in...

In order to make the problem more tractable, we linearize the objective function given in~\eqref{obj:1}. The non-linearity of~\eqref{pb:1} comes from the functions $C(\mathbf{x})$ and $M(\mathbf{x})$ due to the multiplication of binary variables. To linearize $M(\mathbf{x})$, we introduce a new binary variable called $z_{i'i}^k(t)=x_{i'}^k(t-1)x_i^k(t)$. It is clear that this new z-variable is positive if and only if each term of the product of the x-variables is positive. In other words, $z_{i'i}^k(t)=1\iff x_{i'}^k(t-1)=x_i^k(t)=1$. This means that we must add the following two constraints to force the z-variable to be zero whenever $x_{i'}^k(t-1)$ or $x_i^k(t)$ is zero:
\begin{align}\label{cns1_zx1}
    z_{i'i}^k(t)\leq x_{i'}^k(t-1),\forall i,i',k,t>1,
\end{align}
and
\begin{align}\label{cns1_zx2}
    z_{i'i}^k(t)\leq x_{i}^k(t),\forall i,i',k,t.
\end{align}

It remains to enforce the constraints that if both $x_{i'}^k(t-1)$ and $x_i^k(t)$ are equal to one, then the z-variable is one. This can be written as follows:
\begin{align}\label{cns1_zx3}
    z_{i'i}^k(t)\geq x_{i'}^k(t-1)+x_{i}^k(t)-1,\forall i,i',k,t>1.
\end{align}
Thus, the migration cost can be rewritten as follows:
\begin{align}\label{mig_cost2}
    M(\mathbf{z})=\sum_{i=1}^N\sum_{i'=1}^N\sum_{k=1}^K\sum_{t=1}^Tz_{i'i}^k(t)m_{i'i}^k(t),
\end{align}

Now, to linearize $C(\mathbf{x})$, we let $y^k(t)$ denotes the quantity $\sum_{i=1}^Nx_{i}^k(t)n_i(t)\frac{c^k(t)}{f_i}$, i.e.,
\begin{align}\label{y1}
    y^k(t)\coloneqq \sum_{i=1}^Nx_{i}^k(t)n_i(t)\frac{c^k(t)}{f_i},\forall k,t.
\end{align}
Thus, the computing delay $C(\mathbf{y})$ can be rewritten as follows:
\begin{align}\label{comput_delay2}
    C(\mathbf{y})=\sum_{k=1}^K\sum_{t=1}^Ty^k(t).
\end{align}
Now, we have to enforce that the following constraints:
\begin{align}
    x_{i}^k(t)=1 \Rightarrow  y^k(t)=n_i(t)\frac{c^k(t)}{f_i}.
\end{align}
These are indicator constraints that can be easily implemented in the off-the-shelf solvers such as CPLEX or Gurobi. They can be easily transformed to linear constraints using the big-M method.
